Online switching control with stability and regret guarantees

This paper considers online switching control with a finite candidate controller pool, an unknown dynamical system, and unknown cost functions. The candidate controllers can be unstabilizing policies. We only require at least one candidate controller to satisfy certain stability properties, but we do not know which one is stabilizing. We design an online algorithm that guarantees finite-gain stability throughout the duration of its execution. We also provide a sublinear policy regret guarantee compared with the optimal stabilizing candidate controller. Lastly, we numerically test our algorithm on quadrotor planar flights and compare it with a classical switching control algorithm, falsification-based switching, and a classical multi-armed bandit algorithm, Exp3 with batches.

==> sec8_append_simu.tex <==
\section{Simulation details}


\begin{algorithm}
	\caption{Falsification-Based Switching (variant)}	\label{alg: fbs}
	\begin{algorithmic}[1]
		\STATE  	\textbf{Input:}
		Batch length $\tau$,
		Stability parameters $\kappa, \rho, \beta$.
		Assume the policies $\pi_1, \dots, \pi_N$ have been randomly permuted.
		Let $t_0=0$.
		\FOR{Batch $j=0,1, 2, \dots, $}
    		\STATE Terminate the algorithm if $\Pc_j $ is empty.
    		\STATE Initialize $\Pc_{j+1}=\Pc_j$.
    		Select $I_j = \min \{ i \in [N] : \pi_i \in \Pc_j \}$.
    		\FOR{$t=t_j, \dots, \min(t_j+\tau-1, T)$}
        		\STATE	Implement $K_{I_j}$, observe $x_{t+1}$.
        		\IF{$ \|x_{t +1}\|_2>\kappa \rho^{t+1-t_j}\|x_{t_j}\|_2 +\beta w_{\max}$}
        		\STATE 	Set $\Pc_{j+1}=\Pc_j-\{I_j\}$.
        		\STATE \textbf{Break}
        		\ENDIF
    		\ENDFOR
        	\STATE	Let $t_{j+1}=t+1$.
		\ENDFOR
	\end{algorithmic}
\end{algorithm}



Consider a cruise control problem in (Aaron's paper and Richard's book):
$$m\dot v= F_w-F_r+w $$
where $F_w\approx hu$
and $F_r\approx = f_0+f_1v+f_2v^2$.

Consider time discretization $\Delta t=0.01$. The goal is to let the velocity settle around $v_d$. 

Define $e=v-v_d$. The discrete-time dynamics for $e_t$ is
$$ e_{t+1}=e_t + \frac{h\Delta_t}{m} u_t - \frac{\Delta_t}{m} (f_0+f_1(e_t+v_d)+f_2 (e_t+v_d)^2)+ \frac{\Delta_t}{m} w_t$$





Consider three types of controllers: feedback linearization, min-norm policy by a ISS-control Lyapunov function, and PI control.

Suppose the system parameters are known. If they are unknown, we use certainty equivalence.

\nbf{(i) Feedback linearization:} 
$$\pi_{FL}(e_t)=F_r(e_t+v_d)/h -\rho e_t,$$
where $0<\rho\leq 1.$
Notice that the mass $m$ does not affect FL, only $f_0, f_1, f_2$ affects. Further, $f_0$ does not affect the stability, $f_1$ does not affect the linear structure, only errors in $f_2$ will generate nonlinear closed-loop systems.

\nbf{(ii) Min-norm policy by ISS-CLF.} 
Consider an ISS-CLF $V(e)=\|e\|_2$. Notice that
$$V(e_{t+1})\leq V(\bar e_{t+1})+ \frac{\Delta_t}{m}w_{\max},$$
so we only need 
$$V(\bar e_{t+1}) \leq (1-\rho)V(e_t)$$
where $\bar e_{t+1}$ is the next state from $e_t$ when $w_t=0$.

Consider the optimization problem:
\begin{align*}
    \min_{u_t}& \|u_t\|_2\\
    \text{s.t. } & \|e_t + \frac{h\Delta_t}{m} u_t - \frac{\Delta_t}{m} (f_0+f_1(e_t+v_d)+f_2 (e_t+v_d)^2)\|\leq (1-\rho)\|e_t\|
\end{align*}
We can write down the closed-form solution below.
\begin{align*}
    u_t=\begin{cases}
        0 & \text{if } (1-\rho) \|e_t\|\geq \|e_t-\frac{\Delta_t}{m} F_r(e_t+v_d)\|\\
        (1-\rho)\frac{m}{\Delta_t h} \|e_t\|-\frac{m}{\Delta_t h}e_t+\frac{1}{h} F_r(e_t+v_d) & \text{if }(1-\rho) \|e_t\|< e_t-\frac{\Delta_t}{m} F_r(e_t+v_d)\\
       - (1-\rho)\frac{m}{\Delta_t h} \|e_t\|-\frac{m}{\Delta_t h}e_t+\frac{1}{h} F_r(e_t+v_d) &\text{if }(1-\rho) \|e_t\|< -(e_t-\frac{\Delta_t}{m} F_r(e_t+v_d))
    \end{cases}
\end{align*}
Trouble: for $\Delta_t/m\approx 10^{-5}$, this is the same as FL! Hence, we only need to use FL. 
Min-norm is only useful when the nonlinear part is helping you, but here it is harming you.

However, this can be a good example.

\red{however, we can make a robust version with respect to $f_2,f_1, f_0$.}

\nbf{(iii) PID control.} We adopt the approach in (cite?? Richard's feedback control book) to design PID control. We first linearize the system around 0, then design PID with formula in Example 7.8. 



\subsection{Experiment settings.}
\nbf{Parameters:}

\nbf{What to plot?}
Two uncertainties for each unknown parameter $f_0, f_1, f_2$. There are 8 uncertainties. Further, use FL, Robust-CLF, and PID. There are 24 controllers. 


Three experiments:\\
1). we know the parameters, but only compare three controllers (but this case, all are stable, can be boring).\\
2). we don't know the parameters, so some policies are unstable. \\
3). we don't know the parameters, and the true parameter is not in the set, further, there are unmodeled errors,  so some non-robust ones are unstable. 


Trouble: it will be boring if every time we select PID. 




We set $\kappa, \rho, \beta$ very large. We can also increase it if something goes wrong.


\red{How about we say we compare two design methods: feedback linearization, and PID design based on Jacobian linearization?} Say there are of course a lot more methods, e.g., sliding mode, robust control, MRAC, etc. But, here, as an illustration, we only compare two.

We have two types of uncertainties: structured and unstructured. 

Notice that unstructured ones may not be bounded globally, but we still run our algorithm and see what happens.


